Revisiting the Power of Prompt for Visual Tuning

Visual prompt tuning (VPT) is a promising solution incorporating learnable prompt tokens to customize pre-trained models for downstream tasks. However, VPT and its variants often encounter challenges like prompt initialization, prompt length, and subpar performance in self-supervised pretraining, hindering successful contextual adaptation. This study commences by exploring the correlation evolvement between prompts and patch tokens during proficient training. Inspired by the observation that the prompt tokens tend to share high mutual information with patch tokens, we propose initializing prompts with downstream token prototypes. The strategic initialization, a stand-in for the previous initialization, substantially improves performance in fine-tuning. To refine further, we optimize token construction with a streamlined pipeline that maintains excellent performance with almost no increase in computational expenses compared to VPT. Exhaustive experiments show our proposed approach outperforms existing methods by a remarkable margin. For instance, it surpasses full fine-tuning in 19 out of 24 tasks, using less than 0.4% of learnable parameters on the FGVC and VTAB-1K benchmarks. Notably, our method significantly advances the adaptation for self-supervised pretraining, achieving impressive task performance gains of at least 10% to 30%. Besides, the experimental results demonstrate the proposed SPT is robust to prompt lengths and scales well with model capacity and training data size. We finally provide an insightful exploration into the amount of target data facilitating the adaptation of pre-trained models to downstream tasks. The code is available at https://github.com/WangYZ1608/Self-Prompt-Tuning.

==> table/compare_FGVC_sup.tex <==
\begin{table*}[h]
\centering
\caption{\small 
\textbf{Comparisons with previous results on FGVC} with ViT-B pretrained on supervised ImageNet-21K.
We report the average performance (Mean Acc and Params) and per-task results. 
“Input” and “Backbone”indicates the tuning scope of each method.
SPT outperforms competitors with far fewer trainable parameters.}
\vspace{2mm}
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{3.0pt}
\resizebox{1.0\textwidth}{!}{%
    \footnotesize
    \begin{tabular}{l|cccc|ccccc}
        % ~ & \multicolumn{2}{c}{scope} & ~\\
        Methods & Input & Backbone & Params (M) & Mean Acc & CUB-200-2011 & NABirds & Oxford Flowers & Stanford Dogs & Stanford Cars\\
        \hline
        \toprule
        Full & ~ & $\checkmark$ & 85.98 & 88.54 & 87.3 & 82.7 & 98.8 & 89.4 & 84.5\\
        Linear & ~ & ~          & 0.18  & 79.32 & 85.3 & 75.9 & 97.9 & 86.2 & 51.3\\
        \hline
        Bias & ~ & $\checkmark$ & 0.28  & 88.41 & 88.4 & 84.2 & 98.8 & \textbf{91.2} & 79.4\\
        Adapter & ~ & $\checkmark$ & 0.41 & 85.66 & 87.1 & 84.3 & 98.5 & 89.8 & 68.6\\
        MP  & ~ & $\checkmark$  & 1.20 & 89.38 & 89.3 & 84.9 & 99.6 & 89.5 & 83.6\\
        SSF & ~ & $\checkmark$  & 0.39 & 90.72 & 89.5 & 85.7 & 99.6 & 89.6 & 89.2\\
        SNF & ~ & $\checkmark$  & 0.25 & 90.74 & 90.2 & 87.4 & 99.7 & 89.5 & 86.9\\
        \hline
        VPT-shallow & $\checkmark$ & ~ & 0.25 & 84.62 & 86.7 & 78.8 & 98.4 & 90.7 & 68.7\\
        VPT-Deep & $\checkmark$ & ~    & 0.85 & 89.11 & 88.5 & 84.2 & 99.0 & 90.2 & 83.6\\
        E$^2$VPT & $\checkmark$ & ~    & 0.56 & 89.22 & 89.1 & 84.6 & 99.1 & 90.5 & 82.8\\
        \hline
        SPT-Shallow & $\checkmark$ & ~    & 0.25 & 90.10  & 90.2 & 85.1 & 99.5 & 89.3 & 86.4\\
        SPT-Deep & $\checkmark$ & ~    & 0.36    & \textbf{91.40}  & \textbf{90.6} & \textbf{87.6} 
        & \textbf{99.8} & 89.8 & \textbf{89.2}\\
    \end{tabular}
}
\vspace{-1mm}
\label{tab:sota_fgvc_sup}
\end{table*}

==> table/compare_VTAB_sup.tex <==
\begin{table}[t]
\centering
\caption{\small 
\textbf{Comparisons with previous results on VTAB-1K} with ViT-B pretrained on supervised ImageNet-21K.
We report the average accuracy of each group. 
Per-task results presented in Appendix Table.~\ref{tab:appendix_vtab}.}
\vspace{2mm}
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{2.0pt}
\resizebox{0.49\textwidth}{!}{%
    \footnotesize
    \begin{tabular}{l|cccc}
        Methods & Params (M) & \textit{Nature} (7) & \textit{Specialized} (4) & \textit{Structured} (8)\\
        \hline
        \toprule
        Full        & 85.84 & 75.88 & 83.36 & 47.64\\
        Linear      & 0.04 & 68.93 & 77.16 & 26.84\\
        \hline
        Bias        & 0.14 & 73.30 & 78.25 & 44.09\\
        Adapter     & 0.27 & 70.39 & 77.11 & 33.43\\
        LoRA        & 0.32 & 79.49 & 84.55 & \textbf{59.77}\\
        SSF         & 0.24 & 81.57 & \textbf{86.55} & 58.96\\
        SNF         & 0.29 & \textbf{83.78} & 86.13 & 59.61\\
        \hline
        VPT-shallow & 0.11 & 76.81 & 79.68 & 46.98\\
        VPT-Deep    & 0.60 & 78.48 & 82.43 & 54.98\\
        E$^2$VPT    & 0.31 & 80.01 & 84.43 & 57.39\\
        \hline
        SPT-Shallow & 0.11 & 81.44 & 83.65 & 52.86\\
        SPT-Deep    & 0.22 & 82.27 & 85.48 & 58.91\\
    \end{tabular}
}
\vspace{-1mm}
\label{tab:sota_vtab_sup}
\end{table}
